Privacy-Preserving Collaborative Prediction using Random Forests

We study the problem of privacy-preserving machine learning (PPML) for ensemble methods, focusing our effort on random forests. In collaborative analysis, PPML attempts to solve the conflict between the need for data sharing and privacy. This is especially important in privacy sensitive applications such as learning predictive models for clinical decision support from EHR data from different clinics, where each clinic has a responsibility for its patients' privacy. We propose a new approach for ensemble methods: each entity learns a model, from its own data, and then when a client asks the prediction for a new private instance, the answers from all the locally trained models are used to compute the prediction in such a way that no extra information is revealed. We implement this approach for random forests and we demonstrate its high efficiency and potential accuracy benefit via experiments on real-world datasets, including actual EHR data.

==> contents/extra.tex <==
%\begin{wrapfigure}{R}{0.5\textwidth} 
%	\vspace*{-.7cm}
%	\includegraphics[width=\linewidth]{contents/hyperparameters_without_log_rot.png}
%	\caption{Acceptable combinations of maximum depth $d$ and number of trees $m$ such that the model size is at most $2^{13}$.}
%	\label{fig:size_params}
%	\vspace*{-.7cm}
%\end{wrapfigure}

\begin{wrapfigure}{R}{0.4\textwidth} 
	\centering
	\begin{tabular}{lrr}
		Name & Inst. & Feats. \\
		\hline \\
		breast cancer & 569 & 30 \\
		australian & 609 & 14 \\
		colon cancer & 62 & 2,000 \\
		leukemia & 72 & 7,129 \\
		spambase & 4,601 & 57 \\
	\end{tabular}
	\makeatletter\def\@captype{table}\makeatother% "Change float to table"
	\caption{Dataset sizes in instances and features.}
	\label{tab:data}
\end{wrapfigure}


Our approach for tuning the hyperparameters for our random forest model is a constrained gridsearch approach where we consider some reasonably sized subset of $Q_s$, the set of valid hyperparameter choices for a model with maximum nodes $s$.
Through this approach, we maximize the efficacy of our model while respecting the constraints imposed by our encryption algorithm.


%We consider the five different datasets of Table~\ref{tab:data}. and for each one of them we trained a random forest using the learning rule of Appendix~\ref{app:learning} (\Irene{check this! \at \textbf{Yoon, Ross}: is this true?}) implemented via the Scikit-learn library. \Ross{I think that we should remove the ID3 algorithm from the paper unless it is heavily used elsewhere. I do not believe that is the current algorithm used in sklearn and I feel it is reasonable to simply reference the sklearn.}
%Then we run the off-line phase of our system, where the forest is outsourced to the serve, and the on-line phase, where the prediction for a new data point according to the uploaded model is computed.

\begin{table}
	\caption{Overhead our system when the UCI dataset is split among $t$ providers and each of them learns a forest with 50 trees and maximum tree depth $8$.}
	\label{tab:all}   
	\centering
	\setlength{\tabcolsep}{6pt}
	%\footnotesize 
	\renewcommand{\arraystretch}{1.1}
	\begin{tabular}{|l|c|cc|cc|}
		\hline
		\multirow{2}{*}{Dataset}  & \multirow{2}{*}{$t$} &  \multicolumn{2}{c|}{off-line} &  \multicolumn{2}{c|}{on-line} \\
		&                              &             Time (secs)           & Size (MB) &             Time (secs)          & Size (MB)             \\ \hline
		Australian           
		& 2            & 3.02 &  & 0.680  &  \\
		& 4            & 6.67 &  & 0.680  &  \\
		& 6            & 10.10 &  & 0.680  &  \\
		\hline
		Breast cancer        
		& 2            & 0.163 &  & 0.846  &  \\
		& 4            & 0.163 &  & 0.846  &  \\
		& 6            & 0.163 &  & 0.846  &  \\
		\hline
		Colon cancer           
		& 2          & 0.368 &  & 18.874 &  \\
		& 4            & 0.163 &  & 0.846  &  \\
		& 6            & 0.163 &  & 0.846  &  \\
		\hline
		Leukemia
		& 2          & 0.953 &  & 65.530 &\\
		& 4            & 0.163 &  & 0.846  &  \\
		& 6            & 0.163 &  & 0.846  &  \\
		\hline
		Spambase          
		& 2          &  &  &  &\\
		& 4            & 0.163 &  & 0.846  &  \\
		& 6            & 0.163 &  & 0.846  &  \\\hline
	\end{tabular}
\end{table}

%Table~\ref{tab:tree} reports the running time of each step of the core protocol of our system, protocol $\Pte$, when executed of a single tree in function of the parameters $d$ and $n$.
%
%
%\begin{table}
%	\caption{Detailed running time for protocol $\Pte$. \todo{!}}
%	\label{tab:tree}   
%	\begin{center}
%	\setlength{\tabcolsep}{7pt}
%	\footnotesize \renewcommand{\arraystretch}{1.3}
%	\begin{tabular}{|l|c|c|c|c|c|}
%		\hline
%		Dataset &  Step 1 & Step 2 &  Step 3 & Step 4 &  Step 5\\ \hline
%		     
%	\end{tabular}
%
%	\end{center}
%\end{table}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
For a forest with $m$ trees, it is enough to multiply by $n$ the complexity of step 2.
\begin{table}
	\begin{center}
		\caption{Overview of the complexity for protocol $\Ppps$.}
		\label{tab:complexity2} 
		\setlength{\tabcolsep}{4pt}
		\renewcommand{\arraystretch}{1.3}
		\begin{tabular}{|l|c|c|c|c|}
			\hline
			& &\multicolumn{2}{c|}{Computation} & Communication\\\cline{3-4}
			&  & Client & Provider & \\ \hline
			Step 1 & &  $n$ encryptions &  & $n$ ciphertexts\\ \hline
			Step 2 & (a) &   & $(2^d-1)$ $\odot$ & \\ 
			& (c) & $(2^d-1)$ decryptions & $(2^d-1)$  $\odot$  & $(2^d-1)$ ciphertexts \\ 
			& &  & $(2^d-1)$ $\mult$  & \\
			& (e) &$\binom{2^d}{1}$-OT receiver & $\binom{2^d}{1}$-OT sender & $\binom{2^d}{1}$-OT communication \\
			& &			 &  $2^d$ $\odot$ & $2^d$ ciphertexts\\ \hline
			Step 3 & &  $2^d-1$ decryptions & $2^d-1$ $\mult$  & $2^d-1$ ciphertexts\\ 
			&  & 	& $2^d-1$ $\odot$  & \\\hline
		\end{tabular}
	\end{center}  
\end{table}



%%%%%%%%%%%%%%%%%
TREE
	\begin{tikzpicture}[level distance=1cm,
	level 1/.style={sibling distance=2cm},
	level 2/.style={sibling distance=1cm}, scale=0.7]
	\tikzstyle{every node}=[circle,draw, scale=0.7]
	\node (Root)  {$N_1$}
	child{
		node {$N_2$} 
		child { node {$\ell_1$}}
		child { node {$\ell_2$}}	
	}
	child{
		node {$N_3$}
		child { node {$\ell_3$} }
		child { node {$\ell_4$} }
	};	
	\end{tikzpicture}
	
	
	TREE with labels
	
	%\begin{tikzpicture}[level distance=1cm,
	%		level 1/.style={sibling distance=2cm},
	%		level 2/.style={sibling distance=1cm}, scale=0.8]
	%		\tikzstyle{every node}=[circle,draw, scale=0.7]
	%		\node (Root)  {$N_1$}
	%		child{
	%			node[fill=orange!40] {$N_2$}  
	%			child { node[fill=orange!70] {$\ell_1$} edge from parent node[left,draw=none] {$-1$}}
	%			child { node[fill=orange!80!red] {$\ell_2$} edge from parent node[right,draw=none] {$+1$}}
	%			edge from parent node[left,draw=none] {$-1$}	
	%			}
	%			child{
	%				node[fill=blue!20] {$N_3$}
	%					child { node[fill=blue!60] {$\ell_3$} edge from parent node[left,draw=none] {$-1$}}
	%					child { node[fill=blue!80] {$\ell_4$} edge from parent node[right,draw=none] {$+1$}}
	%					edge from parent node[right,draw=none] {$+1$}
	%				};	
	%\end{tikzpicture} 
	
	
HEATMAP
%\begin{figure}
%	\centering
%	\includegraphics[width=\textwidth]{contents/merge_final.png}
%	\caption{Subfigures \textbf{B}-\textbf{F} show how AUC is impacted by the number of providers. The dashed, solid and dotted lines shows AUC values for the locally learn then merge, the zero-sharing and the merge then learn approach, respectively. Subfigure \textbf{A} shows the AUC difference between the locally learn then merge and merge then learn (positive values indicate an improvement using locally learn then merge).}
%	\label{fig:merge}
%\end{figure}
%\input{contents/fig_servers.tex}

